When Natural Strategies Meet Fuzziness and Resource-Bounded Actions (Extended Version)

In formal strategic reasoning for Multi-Agent Systems (MAS), agents are typically assumed to (i) employ arbitrarily complex strategies, (ii) execute each move at zero cost, and (iii) operate over fully crisp game structures. These idealized assumptions stand in stark contrast with human decision making in real world environments. The natural strategies framework along with some of its recent variants, partially addresses this gap by restricting strategies to concise rules guarded by regular expressions. Yet, it still overlook both the cost of each action and the uncertainty that often characterizes human perception of facts over the time. In this work, we introduce HumanATLF, a logic that builds upon natural strategies employing both fuzzy semantics and resource bound actions: each action carries a real valued cost drawn from a non refillable budget, and atomic conditions and goals have degrees in [0,1]. We give a formal syntax and semantics, and prove that model checking is in P when both the strategy complexity k and resource budget b are fixed, NP complete if just one strategic operator over Boolean objectives is allowed, and Delta^P_2 complete when k and b vary. Moreover, we show that recall based strategies can be decided in PSPACE. We implement our algorithms in VITAMIN, an open source model checking tool for MAS and validate them on an adversarial resource aware drone rescue scenario.

==> CameraReady/LaTeX/macros.tex <==
%double quote command
\newcommand\dquote[1]{``#1''}
\newcommand\dquoteit[1]{``\emph{#1}''}

%single quote command
\newcommand\squote[1]{`#1'}


\newif\ifdraft\drafttrue%false


\newcommand{\lexpr}{\ensuremath{\preceq_e}}
\newcommand{\ldist}{\ensuremath{\preceq_d}}

% Abbreviations

\newcommand{\ie}{i.e.}
\newcommand{\eg}{e.g.}
\newcommand{\egdef}{:=}
\newcommand{\colonequals}{:=}
\newcommand{\coloncolonequals}{::=}
\newcommand{\wlogen}{w.l.o.g.\xspace}
\newcommand{\liste}[3]{#1_{#2},\ldots,#1_{#3}}
\newcommand{\bigiff}{\;\;\;iff\;\;\;}

%%%%
% General
\newcommand{\AgSize}{\mathsf{n}} 
\newcommand{\init}{{I}}
\newcommand{\env}{\textsf{e}}
\newcommand{\system}{\textsf{s}}

\newcommand{\dom}{\textit{dom}}
\newcommand{\codom}{\textit{codom}}
\newcommand{\partialto}{\rightharpoonup}
\newcommand{\pref}{\le}
\newcommand{\last}{\mbox{last}}
\newcommand{\FPref}[1]{\textit{pref}\,(#1)}

% Sets

\newcommand{\inter}{\cap}
\newcommand{\union}{\cup}
\newcommand{\dunion}{\uplus}
\newcommand{\biginter}{\bigcap}
\newcommand{\bigunion}{\bigcup}
\newcommand{\compo}{\circ}
\newcommand{\sse}{\subseteq}

%%% Logic

\newcommand{\APf}{\textnormal{Ap}}
\renewcommand{\phi}{\varphi}
\newcommand{\subf}{\textit{Sub}}
\newcommand{\true}{\texttt{true}}
\newcommand{\false}{\texttt{false}}
\newcommand{\ou}{\vee}
\newcommand{\et}{\wedge}
\newcommand{\bigou}{\bigvee}
\newcommand{\biget}{\bigwedge}
\newcommand{\impl}{\to}
\newcommand{\equivaut}{\leftrightarrow}
%\newcommand{\sem}[2]{\llbracket #1 \rrbracket^{#2}}
%\newcommand{\semb}[2][\ltree]{\llbracket #2 \rrbracket^{{#1}}}


% Temporal logic
\newcommand{\Prop}{\APf} %{{Prop}}
\newcommand{\until}{{\bf U}}
\newcommand{\U}{\until\xspace}
\newcommand{\release}{{\bf R}}
\newcommand{\R}{\release}
\newcommand{\wuntil}{\widetilde{\bf U}}
\newcommand{\rond}{\fullmoon}
\newcommand{\X}{{\bf X}}
\newcommand{\G}{{\bf G}}
\newcommand{\F}{{\bf F}}
\newcommand{\trinf}{\pi}
\newcommand{\trfin}{\rho}
\newcommand{\E}{{\bf E}}
\newcommand{\A}{{\bf A}}

%% SL

\newcommand{\Var}{\textnormal{Var}} 
\newcommand{\var}{s}
\newcommand{\varb}{t}
\newcommand{\Estrat}[1][\var]{\exists #1.\,}
\newcommand{\Astrat}[1][\var]{\forall #1.\,}
\newcommand{\Estrata}[2][\var]{\exists #1_{#2}.\,}
\newcommand{\Astrata}[2][\var]{\forall #1_{#2}.\,}
\newcommand{\bind}[2][\ag]{(#1,#2)}
\newcommand{\emptystrat}{\unb}
\newcommand{\unbind}[1][\ag]{(#1,\unb)}
\newcommand{\Aout}{{\bf A}}
\newcommand{\Eout}{{\bf E}}

\newcommand{\Ka}[1][\ag]{K_{#1}}

\newcommand{\freeFun}[1]{\free(#1)}

%% ATL
\newcommand{\coop}[1]{\langle\!\langle{#1}\rangle\!\rangle}
\newcommand{\noavoid}[1]{[\![{#1}]\!]}
\newcommand{\coalition}{A}
\newcommand{\coopobs}[1]{\coop{#1}^\bullet} \newcommand{\coal}[1]{[{#1}]} \newcommand{\coopcl}[1]{\ensuremath{[#1]}}


%% New operators

\newcommand{\does}[2]{\text{does}(#1,#2)}
\newcommand{\rational}[2]{\text{rat}(#1,#2)}

\newcommand{\objassign}{\Omega}


%% Concurrent game structures
\newcommand{\consume}{consume}

\newcommand{\Ag}{\textnormal{Ag}}
\newcommand{\ag}{a}
\newcommand{\agb}{b}
\newcommand{\Act}{\textnormal{Act}}
\newcommand{\Mov}{\Act}
\newcommand{\setmoves}{\Mov}
\newcommand{\maxmov}{l}
\newcommand{\act}{c}
\newcommand{\mov}{\act}
\newcommand{\mova}[1][\ag]{\mov_{#1}}
\newcommand{\jmov}{\profile{\mov}}
\newcommand{\setpos}{St}
\newcommand{\sethistory}{H}
\newcommand{\settree}{T}
\newcommand{\pos}{st}
\newcommand{\CGS}{\relax\ifmmode\mathcal G\else$\textrm{CGS}$\xspace\fi}
\newcommand{\trans}{\delta}
\newcommand{\transCGS}{t}
\newcommand{\availability}{d}
\newcommand{\val}{\ell}
\newcommand{\fplay}{\rho}
\newcommand{\iplay}{\pi}
\newcommand{\hist}{h}
\newcommand{\strat}{\sigma}
\newcommand{\out}{\textnormal{out}}
\newcommand{\FPlay}{\text{Plays}}
\newcommand{\eqc}[2][\pos]{[#1]_{#2}}

%mie
\newcommand{\Agt}{\mathbb{A}\textnormal{gt}}
\newcommand{\dual}[1]{\llbracket {#1} \rrbracket}

\newcommand{\INDSTATE}[1][1]{\STATE\hspace{#1\algorithmicindent}}

\newcommand{\set}[1]{\{#1\}}
\newcommand{\setstrat}{\mbox{\emph{Str}}}
\newcommand{\setstrata}[1][\ag]{\mbox{\emph{Str}}_{#1}}
\newcommand{\setstrats}[1][\pos]{\mbox{\emph{Str}}(#1)}
\newcommand{\assign}{\mathcal A}%{\chi}

\newcommand{\obsrel}[1][\ag]{\sim_{#1}}

\newcommand{\verf}{\text{v}}
\newcommand{\reft}{\text{r}}
\newcommand{\memoryless}{\text{r}}
\newcommand{\perfectrecall}{\text{R}}
\newcommand{\imperfectinfo}{\text{i}}
\newcommand{\perfectinfo}{\text{I}}

\newcommand{\setting}{\rho}

\newcommand{\myi}{{(i)}\xspace}
\newcommand{\myii}{{(ii)}\xspace}
\newcommand{\myiii}{{(iii)}\xspace}
\newcommand{\myiv}{{(iv)}\xspace}
\newcommand{\myv}{{(v)}\xspace}
\newcommand{\myvi}{{(vi)}\xspace}

%% Quantitative SL

\newcommand{\wCGS}{\relax\ifmmode \mathcal G\else$\textrm{wCGS}$\xspace\fi}
\newcommand{\rfCGS}{\relax\ifmmode \mathcal G\else$\textrm{rfCGS}$\xspace\fi}
\newcommand{\wCGT}{\relax\ifmmode \mathcal T\else$\textrm{wCGT}$\xspace\fi}
\newcommand{\Module}{\mathcal M}
\newcommand{\semSLgeneral}[4][]{\llbracket #4 \rrbracket^{#1}_{#2}(#3)}
\newcommand{\semSL}[4][\wCGS]{\llbracket #4 \rrbracket^{#1}_{#2}(#3)}
\newcommand{\denotation}[2][]{\llbracket #2 \rrbracket^{#1}}
\newcommand{\semSLglobal}[2][\wCGS]{\llbracket #2 \rrbracket^{#1}}
\newcommand{\RsemSL}[4]{\llbracket #4 \rrbracket^{#1}_{#2}(#3)}
\newcommand{\RsemglobalSL}[2]{\llbracket #2 \rrbracket^{#1}_{#2}}
\newcommand{\pred}{P}
\renewcommand{\Gamma}{A}
\renewcommand{\sigma}{s}
\newcommand{\react}{r}
\newcommand{\modelchk}{\models_{\pred}}
\newcommand{\modulechk}{\models_{\pred}^{\react}}
\newcommand{\unwinding}{\mthfun{Unw}}
\newcommand{\exec}{\mthfun{exec}}


%% Trees
\newcommand{\Dirtree}{X}
\newcommand{\dir}{x}
\newcommand{\dira}{y}
\newcommand{\dirz}{z}
%\newcommand{\racine}{r}
\renewcommand{\root}{r}
\newcommand{\node}{u}
\newcommand{\nodeb}{v}
%\newcommand{\noeudb}{w}
\newcommand{\setnodes}{U}
\newcommand{\tree}{T} %\newcommand{\tree}{\tau}
\newcommand{\ltree}{t}
\newcommand{\lab}{\ell}
\newcommand{\plab}[1][p]{\ell_{#1}}
\newcommand{\prodlab}{\otimes}
\newcommand{\Dir}{\mbox{\textit{Dir}}}
\protected\def\tpath{\ifmmode \spath \else path\xspace\fi}
\newcommand{\tpaths}{paths\xspace}
\newcommand{\tPaths}{Paths}

\newcommand{\Hist}{\ensuremath{\mathrm{\textup{Hist}}}\xspace}

\newcommand{\Br}[1]{\text{Br}(#1)}

%% Kripke structures
\newcommand{\struct}{\mathcal S}
\newcommand{\KS}{\relax\ifmmode \struct\else\textrm{wKS}\xspace\fi}
%\newcommand{\wKS}{\textrm{wKS}\xspace}
\newcommand{\setstates}{S}
\newcommand{\sstate}{s}
\newcommand{\relation}{R}
\newcommand{\spath}{\lambda}
\newcommand{\Paths}{\text{Paths}}
\newcommand{\FPaths}{\text{FinPaths}}
\newcommand{\Pequiv}[1][p]{\equiv_{#1}}

\newcommand{\unfold}[2][\KS]{\ltree_{#1}}
\newcommand{\domunfold}[2][\KS]{\tree_{#1}(#2)}
\newcommand{\labunfold}[2][\KS]{\lab_{#1}(#2)}


%% QCTL
\newcommand{\existsp}[1][p]{\exists #1.\,}
\newcommand{\forallp}[2][p]{\forall #1.\,}
\newcommand{\modelss}{\models_s}
\newcommand{\modelst}{\models}
\newcommand{\uniq}[1][p]{\mathrm{uniq}(#1)}

%% QCTL[F]
\newcommand{\setvaltext}{\textup{Val}}
\newcommand{\setval}[1]{\setvaltext_{#1}}
\newcommand{\approxsetval}[1]{\widetilde{\setvaltext}_{#1}}
\newcommand{\values}{\mathcal V}
\newcommand{\sem}[3][\ltree]{\llbracket #2 \rrbracket^{{#1}}(#3)}
\newcommand{\semb}[2][\ltree]{\llbracket #2 \rrbracket^{{#1}}}
\newcommand{\Bool}{\text{Bool}}


%% Tree automata
\newcommand{\boolp}{\mathbb B^+}
\newcommand{\tauto}{\mathcal A}
\newcommand{\Nauto}{\ifmmode \mathcal N \else NPT\xspace\fi}
\newcommand{\Uauto}{\ifmmode \mathcal U \else UPT\xspace\fi}
\newcommand{\tQ}{Q}
\newcommand{\tQp}{\tQ^\top}
\newcommand{\tQm}{\tQ^\perp}
\newcommand{\tq}{q}
\newcommand{\tDelta}{\Delta}
\newcommand{\tdelta}{\delta}
\newcommand{\proj}[2][p]{\begingroup #2\!\Downarrow^{\exists}_{#1}\endgroup}
\newcommand{\proju}[2][p]{\begingroup #2\!\Downarrow^{\forall}_{#1}\endgroup}
\newcommand{\auto}{\ifmmode \tauto \else APT\xspace\fi}
\newcommand{\couleur}{C}
\newcommand{\wauto}{\mathcal W}
\newcommand{\Automaton}{\auto}
\newcommand{\Language}{\mathcal L}
\newcommand{\game}{G}
\newcommand{\tgame}[3]{\game(#1,#2,#3)}
\newcommand{\automc}[3][\values]{\auto^{#1,#2}_{#3}}
\newcommand{\ndepth}{\mathrm{nd}}



%% Reduction

\newcommand{\APq}{{\APf_{\exists}}}
\newcommand{\APS}{\APf_{\CKS}}
\newcommand{\APfree}{\APf_{f}}
\newcommand{\blank}{\mathbf{0}}
\newcommand{\labS}{\lab_\CKS}
\newcommand{\APm}{\APf_{\mov}}
\newcommand{\APv}{\APf_{\pos}}
\newcommand{\tr}[2][f]{(#2)_{\mathrm{s}}^{\,#1}} 
\newcommand{\trp}[2][f]{(#2)_{\mathrm{p}}^{\,#1}} 
\newcommand{\phistrat}[1][\var]{\phi_{\text{str}}(#1)}
\newcommand{\psistrat}[1][\var]{\psi_{\text{str}}^{#1}}
\newcommand{\psistratdet}[1][\var]{\psi_{\text{str,det}}^{#1}}
\newcommand{\phistratdet}[1][\var]{\phi_{\text{str}}^{\text{det}}(#1)}
\newcommand{\phiout}[1][\assign]{\Phi_{\text{out}}^{\,#1}}
\newcommand{\psiout}[1][\Vtrad]{\psi_{\text{out}}^{\,#1}}
\newcommand{\phiturn}{\phi_{\text{tb}}}


% Names Logics
\newcommand\LTL{\textnormal{\sffamily LTL}\xspace}
\newcommand\LTLs{\ensuremath{\textnormal{{\sffamily LTL}}^{*}}\xspace}
\newcommand\CTL{\textnormal{{\sffamily CTL}}\xspace}
\newcommand\CTLs{\ensuremath{\textnormal{{\sffamily CTL}}^{*}}\xspace}
\newcommand\ATL{\textnormal{{\sffamily ATL}}\xspace}
\newcommand\NatATL{\textnormal{{\sffamily NatATL}}\xspace}
\newcommand\NatATLr{\textnormal{{\sffamily NatATL}}_{\textnormal{r}}\xspace}
\newcommand\NatATLR{\textnormal{{\sffamily NatATL}}_{\textnormal{R}}\xspace}

\newcommand\ATLr{\textnormal{{\sffamily ATL}}_{\textnormal{r}}\xspace}
\newcommand\ATLR{\textnormal{{\sffamily ATL}}_{\textnormal{R}}\xspace}


\newcommand\ATLs{\ensuremath{\textnormal{{\sffamily ATL}}^{*}}\xspace}
\newcommand\ATLsc{\ensuremath{\textnormal{{\sffamily ATL}}_{\text{sc}}}\xspace}
\newcommand\QCTLs{\ensuremath{\textnormal{{\sffamily QCTL}}^{*}}\xspace}
\newcommand{\BQCTL}{\ensuremath{\textnormal{\sffamily{BQCTL}}}\xspace}
\newcommand{\BQCTLs}{\ensuremath{\textnormal{\sffamily{BQCTL}}^{*}}\xspace}
\newcommand\SL{\textnormal{{\sffamily SL}}\xspace}
\newcommand{\Fu}[2]{\ensuremath {{#1}{[#2]}}\xspace}
\newcommand{\Func}{\ensuremath{\mathcal F}}
\newcommand{\LTLF}{\Fu{\LTL}{\Func}}
\newcommand{\CTLsf}{\Fu{\CTLs}{\Func}}
\newcommand{\SLF}{\Fu{\SL}{\Func}}
\newcommand{\ATLF}{\Fu{\ATL}{\Func}}
\newcommand{\NatATLF}{\Fu{\NatATL}{\Func}}
\newcommand{\NatATLrF}{\Fu{\NatATLr}{\Func}}
\newcommand{\NatATLRF}{\Fu{\NatATLR}{\Func}}
\newcommand{\CTLF}{\Fu{\CTL}{\Func}}

\newcommand{\ResNatATLF}{%
  \textnormal{\sffamily Human}\Fu{\NatATL}{\Func}%
}

\newcommand{\ResNatATLrF}{%
  \textnormal{\sffamily Res}\Fu{\NatATLr}{\Func}%
}
\newcommand{\ResNatATLRF}{%
  \textnormal{\sffamily Res}\Fu{\NatATLR}{\Func}%
}

\newcommand{\HumanATLF}{%
  \textnormal{\sffamily Human}\Fu{\ATL}{\Func}%
}

\newcommand{\HumanATLrF}{%
  \textnormal{\sffamily Human}\Fu{\ATLr}{\Func}%
}

\newcommand{\HumanATLRF}{%
  \textnormal{\sffamily Human}\Fu{\ATLR}{\Func}%
}

\newcommand{\ATLsF}{\Fu{\ATLs}{\Func}}

\newcommand{\SLKF}{\Fu{\textnormal{{\sffamily SLK}}}{\Func}}
\newcommand{\SLK}{\textnormal{{\sffamily SLK}}\xspace}
\newcommand{\QCTLsf}[1][\Func]{\Fu{\QCTLs}{#1}}
\newcommand{\BQCTLf}[1][\Func]{\Fu{\BQCTL}{#1}}
\newcommand{\BQCTLsf}[1][\Func]{\Fu{\BQCTLs}{#1}}
\newcommand{\BQCTLsftitle}{\Fu{\BQCTLs}{\Func}}

\newcommand{\Lsys}{\ensuremath{\mathcal{L}}}

% Misc

\newcommand{\free}{\text{free}}
\newcommand{\profile}[1]{\boldsymbol{#1}}
\newcommand{\EFF}{\text{Eff}}
\newcommand{\smv}{\text{smv}}
\newcommand{\sndmax}{2\textrm{nd-max}}
\newcommand{\phismv}{\phi^{\smv}}
\newcommand{\lowb}{0}%%%{-1} %%% -1
\newcommand{\buchi}{B\"{u}chi\xspace}


%% Complexity classes

\protected\def\PTIME{\ifmmode \mbox{\sc P} \else {\sc P}\xspace\fi}
\protected\def\PSPACE{\ifmmode \mbox{\sc Pspace} \else {\sc Pspace}\xspace\fi}
\protected\def\EXPTIME{\ifmmode \mbox{\sc Exptime} \else {\sc Exptime}\xspace\fi}
\protected\def\NONELEMENTARY{\ifmmode \mbox{\sc NonElementary} \else {\sc NonElementary}\xspace\fi}
\protected\def\ELEMENTARY{\ifmmode \mbox{\sc Elementary} \else {\sc Elementary}\xspace\fi}


%% Environments

%\theoremstyle{definition}

% \theoremstyle{plain}
% \newtheorem{property}{Property}
% \newtheorem{proposition}{Proposition}
% %\newtheorem{theorem}{Theorem}
% \newtheorem{corollary}{Corollary}
% \newtheorem{lemma}{Lemma}
% %\theoremstyle{remark}
% \newtheorem{remark}{Remark}
%\newtheorem{example}{Example}

% \newenvironment{proofsketch}[1][Proof sketch]{\par
%   %\pushQED{\qed}%
%   \normalfont \topsep6\p@\@plus6\p@\relax
%   \trivlist
%   \item[\hskip\labelsep
%   %      \color{darkgrey}\sffamily\bfseries
%     \emph{#1}\@addpunct{.}]\ignorespaces
% }{%
%   \endtrivlist%\@endpefalse
% }

\newcommand{\halfline}{\vspace{.5\baselineskip}}
\newcommand{\head}[1]{\noindent \textbf{#1}}
\renewcommand{\ldots}{...}
\renewcommand{\dots}{...}


% Ridifinizione dei comandi per l'ambiente pseudocodice
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}


\algnewcommand\algorithmicguess{\textbf{Guess}}
\algnewcommand\algorithmicendguess{\textbf{EndGuess}}
\algblock{Guess}{EndGuess}


==> CameraReady/LaTeX/sections/07-Discussion.tex <==
\section{\uppercase{Discussion}}
\label{sec:discussion}

\HumanATLF\ captures the essential human tendency to extract simple actionable patterns from the foggy reality in which we are immersed, transforming complexity into a simplified representation \cite{hjeij2023brief}. 

While extending this formalization with knowledge operators, belief systems, strategic hierarchies, and other refinements would enhance its psychological realism, such additions would substantially increase computational complexity.

The primary challenge for future research lies in developing methods to manage this computational burden while preserving expressivity. 

Technically, by defining \HumanATLF\ for human-like representation of strategies, we established a quantitative logic capable of capturing the fuzzy achievement of goals under non‑refillable resource budgets in the context of strategic reasoning in Multi‑Agent Systems. Echoing the landmark results of Natural Strategic Ability \cite{JMM19a}, our analysis builds directly on that foundation, advancing it with a more expressive framework that remains computationally grounded. By reformulating human‑like strategies to account for finite resources, we introduce an explicit bound $b$. Although this refinement does not alter the worst‑case complexity classification, in practice this parameter constrains the space of admissible strategies and thereby reduces the state space of the pruned model during the \HumanATLF\ verification phase.  However, we acknowledge that the combinatorial complexity inherent in any exhaustive strategy generator remains a significant practical limitation, restricting its applicability to relatively simple scenarios when emulating human‑like decision making. Furthermore, our current framework does not prescribe a mechanism for resolving conflicts among ordered condition‑action pairs.  In both memoryless and recall-based approaches, where each condition evaluates to a real value in \([0,1]\), there is no intrinsic rule for selecting which action to execute when multiple conditions hold simultaneously. At present, actions are associated with conditions via a Cartesian product in an effectively random and egalitarian fashion, since we have not yet implemented a priority queue or ranking scheme. In future work, we intend to explore the integration of a priority‑based action selection mechanism to address this issue. Finally, while we present model‑checking results that highlight the theoretical efficacy of our approach, the strategy generator remains primarily a planning prototype; its extension to large‑scale or real‑time applications will require further optimization and empirical validation.

